A robust adaptive model predictive control framework for nonlinear uncertain systems

In this paper, we present a tube-based framework for robust adaptive model predictive control (RAMPC) for nonlinear systems subject to parametric uncertainty and additive disturbances. Set-membership estimation is used to provide accurate bounds on the parametric uncertainty, which are employed for the construction of the tube in a robust MPC scheme. The resulting RAMPC framework ensures robust recursive feasibility and robust constraint satisfaction, while allowing for less conservative operation compared to robust MPC schemes without model/parameter adaptation. Furthermore, by using an additional mean-squared point estimate in the objective function the framework ensures finite-gain $\mathcal{L}_2$ stability w.r.t. additive disturbances. As a first contribution we derive suitable monotonicity and non-increasing properties on general parameter estimation algorithms and tube/set based RAMPC schemes that ensure robust recursive feasibility and robust constraint satisfaction under recursive model updates. Then, as the main contribution of this paper, we provide similar conditions for a tube based formulation that is parametrized using an incremental Lyapunov function, a scalar contraction rate and a function bounding the uncertainty. With this result, we can provide simple constructive designs for different RAMPC schemes with varying computational complexity and conservatism. As a corollary, we can demonstrate that state of the art formulations for nonlinear RAMPC are a special case of the proposed framework. We provide a numerical example that demonstrates the flexibility of the proposed framework and showcase improvements compared to state of the art approaches.

==> Approaches.tex <==
%!TEX root = ./Adaptive_Nonlin.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Design procedure and overall algorithm}
\label{sec:design}
\JK{a different title may be good..., maybe Sec.~IV in Section III (might make more sense)}
Section~\ref{sec:design_1} provides explicit design procedures and the overall algorithm.
%Let Assumptions~\ref{ass:model}, \ref{ass:nominal}, \ref{ass:increm}, \ref{ass:w_tilde} and \ref{ass:term} hold.
%To this end, consider the following additional restrictions:
%\begin{assumption}
%\label{ass:design_assumption}
%Assumption~\ref{ass:model} holds with some polytope $\mathbb{D}$, i.e. $\mathbb{D}=\{d\in\mathbb{R}^q|~H_w d\leq h_w\}$.
%
%Assumption~\ref{ass:increm} holds with a quadratic incremental Lyapunov function $V_{\delta}$, i.e. $V_{\delta}(x,z)=\|x-z\|_P$. 
%\end{assumption}
%Explicit design procedures are introduced in Section~\ref{sec:main_5}. 
%The overall algorithm is summarized in Section~\ref{sec:}. 
In Section~\ref{sec:special_guay} we demonstrate that state of the art approaches~\cite{adetola2011robust,guay2015robust,gonccalves2016robust} are contained as a special case of the proposed formulation. 
Section~\ref{sec:main_6} discusses some extensions and open issues.
%design - algorithms
\input{Approaches_1} 
%\newpage
\input{Approaches_2} 
%\newpage
%extensions
\input{Theory_6}











==> Plots/ClosedLoopAnalysis.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=50,
xlabel style={font=\color{white!15!black}},
xlabel={Time Iterations},
ymin=-0.1,
ymax=0.1,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{State x}_\text{1}$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red]
  table[row sep=crcr]{%
0	0.1\\
1	0.039979\\
2	-0.01575\\
3	-0.051878\\
4	-0.071431\\
5	-0.081834\\
6	-0.086321\\
7	-0.086502\\
8	-0.083329\\
9	-0.078112\\
10	-0.071452\\
11	-0.064155\\
12	-0.056624\\
13	-0.048962\\
14	-0.041643\\
15	-0.034834\\
16	-0.02865\\
17	-0.023108\\
18	-0.018241\\
19	-0.014075\\
20	-0.01054\\
21	-0.0076076\\
22	-0.0051883\\
23	-0.0032789\\
24	-0.0017458\\
25	-0.0006101\\
26	0.00025016\\
27	0.0008395\\
28	0.0012513\\
29	0.0014776\\
30	0.0016071\\
31	0.00162\\
32	0.0015846\\
33	0.0014856\\
34	0.0013043\\
35	0.0011868\\
36	0.0010623\\
37	0.00092793\\
38	0.00081704\\
39	0.00068651\\
40	0.00058654\\
41	0.00047186\\
42	0.00039549\\
43	0.000305\\
44	0.00024982\\
45	0.0001793\\
46	0.00014393\\
47	9.1333e-05\\
48	7.1504e-05\\
49	3.4855e-05\\
50	2.4453e-05\\
};
\addlegendentry{Non-Adaptive Closed-Loop Trajectory}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0	0.1\\
1	0.039979\\
2	-0.012345\\
3	-0.047988\\
4	-0.067986\\
5	-0.079378\\
6	-0.08475\\
7	-0.085467\\
8	-0.082923\\
9	-0.078164\\
10	-0.071898\\
11	-0.064896\\
12	-0.057452\\
13	-0.050038\\
14	-0.042804\\
15	-0.036032\\
16	-0.029795\\
17	-0.024193\\
18	-0.019253\\
19	-0.01499\\
20	-0.011346\\
21	-0.00833\\
22	-0.0058225\\
23	-0.0038147\\
24	-0.0021981\\
25	-0.00096731\\
26	-1.3626e-05\\
27	0.00064722\\
28	0.0011521\\
29	0.0014233\\
30	0.0015817\\
31	0.0016197\\
32	0.0016083\\
33	0.0015238\\
34	0.001428\\
35	0.0012865\\
36	0.0011585\\
37	0.0010038\\
38	0.00087609\\
39	0.00073369\\
40	0.0006265\\
41	0.00050302\\
42	0.00041382\\
43	0.0003158\\
44	0.00025345\\
45	0.00017922\\
46	0.0001389\\
47	8.4739e-05\\
48	6.2553e-05\\
49	2.4598e-05\\
50	1.5975e-05\\
};
\addlegendentry{First Adaptive Closed-Loop Trajectory}

\addplot [color=blue, dashdotted]
  table[row sep=crcr]{%
0	0.1\\
1	0.039979\\
2	-0.014098\\
3	-0.048118\\
4	-0.068421\\
5	-0.079602\\
6	-0.084659\\
7	-0.084729\\
8	-0.083398\\
9	-0.078456\\
10	-0.072042\\
11	-0.064921\\
12	-0.057401\\
13	-0.049924\\
14	-0.042651\\
15	-0.035855\\
16	-0.029608\\
17	-0.024015\\
18	-0.019078\\
19	-0.014823\\
20	-0.01119\\
21	-0.0081886\\
22	-0.0056969\\
23	-0.0037048\\
24	-0.0021035\\
25	-0.00088677\\
26	5.3334e-05\\
27	0.00066774\\
28	0.0011434\\
29	0.001427\\
30	0.001594\\
31	0.0016374\\
32	0.0016287\\
33	0.0015462\\
34	0.0014515\\
35	0.0013097\\
36	0.0011807\\
37	0.0010283\\
38	0.00089741\\
39	0.000752\\
40	0.00064461\\
41	0.0005168\\
42	0.00042619\\
43	0.00032701\\
44	0.00026117\\
45	0.0001847\\
46	0.00014242\\
47	8.6658e-05\\
48	6.3345e-05\\
49	2.4604e-05\\
50	1.5383e-05\\
};
\addlegendentry{Last Adaptive Closed-Loop Trajectory}

\end{axis}
\end{tikzpicture}%
